Human Perception of Audio Deepfakes

The recent emergence of deepfakes has brought manipulated and generated content to the forefront of machine learning research. Automatic detection of deepfakes has seen many new machine learning techniques, however, human detection capabilities are far less explored. In this paper, we present results from comparing the abilities of humans and machines for detecting audio deepfakes used to imitate someone's voice. For this, we use a web-based application framework formulated as a game. Participants were asked to distinguish between real and fake audio samples. In our experiment, 472 unique users competed against a state-of-the-art AI deepfake detection algorithm for 14912 total of rounds of the game. We find that humans and deepfake detection algorithms share similar strengths and weaknesses, both struggling to detect certain types of attacks. This is in contrast to the superhuman performance of AI in many application areas such as object detection or face recognition. Concerning human success factors, we find that IT professionals have no advantage over non-professionals but native speakers have an advantage over non-native speakers. Additionally, we find that older participants tend to be more susceptible than younger ones. These insights may be helpful when designing future cybersecurity training for humans as well as developing better detection algorithms.

==> fig3.tex <==

\begin{figure}
    % \centering
    %  \begin{subfigure}[b]{0.45\textwidth}
    %      \centering
    %      \includegraphics[width=0.99\textwidth]{res/auto_created/user_acc_by_attack_id.png}
    %      \caption{\textbf{User accuracy per attack}.
    %      This graph shows the human players' accuracy, averaged over all \input{res/auto_created/unique_users.txt}users and all \input{res/auto_created/number_of_rounds_played.txt}rounds played, grouped by attack ID. While all of the attacks fool humans to various degrees, attack $A10$ proves to be the most challenging by far.}
    %      \label{fig:userAccuracyPerAttack}
    %  \end{subfigure}
    %  \hfill
    %  \begin{subfigure}[b]{0.45\textwidth}
    %      \centering
    %      \includegraphics[width=0.99\textwidth]{res/auto_created/ml_acc_by_attack_id.png}
    %      \caption{\textbf{Accuracy of the artificial intelligence per attack}.

    %      While the AI performs well for both the benign samples and most of the attacks, $A17$ is extremely challenging to detect for the AI.}
    %      \label{fig:AIAccuracyPerAttack}
    %  \end{subfigure}
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[width=0.99\textwidth]{res/auto_created/both_acc_by_attack_id.png}
         \caption{\textbf{Mean attack accuracy}.
         This graph shows the mean attack accuracy per attack ID (with '-' denoting no attack, i.e. bona-fide samples).
         The blue bars indicate the accuracy of the human players, the green bars indicate the accuracy of the AI (RawNet2).}
        %  While the AI performs well for both the benign samples and most of the attacks, $A17$ is extremely challenging to detect for the AI.}
         \label{fig:AIandHumanAccuracyPerAttack}
     \end{subfigure}
     %\hfill
     \begin{subfigure}[c]{0.45\textwidth}
         \centering
         \includegraphics[width=0.99\textwidth]{res/auto_created/delta_acc_ai_human.png}
         \caption{\textbf{Difference between AI and Human Accuracy}.
         This graph shows the difference between AI and human accuracy. A bar with positive value indicates superior performance of the AI w.r.t.\ a given attack ID.
         Humans and AI perform similarly.
        %  The AI outperforms the human player for all attack except for $A17$, which is known to be challenging~\cite{tak2021end}.
        }
         \label{fig:delta_acc}
     \end{subfigure}
    \caption{Detection performance of participants and the AI.}
    \label{fig:accuracyPerAttack}
\end{figure}

==> res/auto_created/age_divide.tex <==
22

==> res/auto_created/engl_is.tex <==
\begin{tabular}{lr}
\toprule
{} &  Unique User IDs \\
English is a Mother Tongue &                  \\
\midrule
False                      &              367 \\
True                       &              105 \\
\bottomrule
\end{tabular}


==> res/auto_created/location.tex <==
\begin{tabular}{lr}
\toprule
Empty DataFrame
Columns: Index(['Unique User IDs'], dtype='object')
Index: Index([], dtype='object', name='Location') \\
\bottomrule
\end{tabular}


==> res/auto_created/number_of_rounds_played.tex <==
14912

==> res/auto_created/ranges.tex <==
(0, 5), (5, 10), (10, 15), (15, 20) and (20, 25)

==> res/auto_created/rolling_size.tex <==
10

==> res/auto_created/skill2.tex <==
\begin{tabular}{lr}
\toprule
{} &  Unique User IDs \\
Skill Level &                  \\
\midrule
1           &               11 \\
2           &               25 \\
3           &               52 \\
4           &               84 \\
5           &               61 \\
\bottomrule
\end{tabular}


==> res/auto_created/unique_users.tex <==
472
